Fillet-based RRT*: A Rapid Convergence Implementation of RRT* for Curvature Constrained Vehicles

Rapidly exploring random trees (RRTs) have proven effective in quickly finding feasible solutions to complex motion planning problems. RRT* is an extension of the RRT algorithm that provides probabilistic asymptotic optimality guarantees when using straight-line motion primitives. This work provides extensions to RRT and RRT* that employ fillets as motion primitives, allowing path curvature constraints to be considered when planning. Two fillets are developed, an arc-based fillet that uses circular arcs to generate paths that respect maximum curvature constraints and a spline-based fillet that uses Bezier curves to additionally respect curvature continuity requirements. Planning with these fillets is shown to far exceed the performance of RRT* using Dubin's path motion primitives, approaching the performance of planning with straight-line path primitives. Path sampling heuristics are also introduced to accelerate convergence for nonholonomic motion planning. Comparisons to established RRT* approaches are made using the Open Motion Planning Library (OMPL).

==> common_procedures.tex <==
%%
% @File: common_procedures.tex
% @Date: August 2020
% @Author: James Swedeen
%
% @brief
% Define common procedures.
%%

\subsection{Common Sampling-based Planning Procedures}
The literature on sample-based planning defines planning algorithms using a number of procedures.
We now define several generic procedures that can be found in \cite{Karaman2011} with notation changed to match the sequel.

\Procedure{$T \leftarrow Initialize(x_{r})$}
Returns an initialized tree with $x_{r} \in \mathbb{R}^d$ as the root node and no edges, i.e. $T \leftarrow \{V,E\}$, $V \leftarrow \{x_{r}\}$, and $E \leftarrow \varnothing$.

\Procedure{$x_{rand} \leftarrow Sample(X_{s})$}
\label{procedure:sample}
Returns a random state from the set $X_{s} \subset X$.
%Returns a random point from the state set $X_{s} \subset X_{free}$\footnote{Because it is computationally expensive to uniformly sample an arbitrary set, all of $X$ is sampled instead and the sample is discarded if it happens to be in the obstacle set.}.
The sampling is an independent, identically, and uniformly distributed (i.i.u.d.) sample of $X_{s}$\footnote{It is important that the sampling of $X_{s}$ is i.i.u.d. to guarantee asymptotic optimality \cite{Karaman2011}.}.

\Procedure{$x_{nearest} \leftarrow Nearest(x_{rand},T)$}
Finds the nearest vertex in the set $V$ to the state $x_{rand} \in X$ using the 2-norm as a distance.

\Procedure{$X_{near} \leftarrow Near_{\rho,\alpha}(x_{rand},T)$}
Finds the nearest $\alpha \in \mathbb{Z}_+$ vertices that are within a given radius, $\rho \in \mathbb{R}_+$, of the point $x_{rand} \in X$, %i.e.
%\begin{equation*}
%  Near_{\rho,\alpha}(x_{rand},T=\{V,E\}) := \{ v \in V | \rho \geq \| x_{rand} - v \| \},
%\end{equation*}
where $\alpha$ is a constant that prevents too many connections from being attempted in a given iteration \cite{Lavalle2006}.
In this work $\rho$ is held constant, but there are extensions to RRT* based algorithms that vary $\rho$ \cite{Karaman2011}.

\Procedure{$x_{n} \leftarrow Steer_\eta(x,y)$}
\label{procedure:steer}
Returns a point that is within a predefined distance $\eta \in \mathbb{R}_+$ from $x \in X$ in the direction of $y \in X$, i.e.
\begin{equation*}
  Steer_\eta(x,y) := argmin_{\{z \in X | \|z - x \| \leq \eta\}} \|z - y\|
\end{equation*}
The Steer function prevents long edges from being added to RRT search trees.
This is important because it reduces the expected extension length at each iteration and likewise reduces the probability that a given iteration will fail to expand the search tree due to it's edge being blocked by an obstacle \cite{lan2015}.

\Procedure{$T \leftarrow InsertNode(x_{n},x_{p},T)$}
Adds the node $x_{n} \in X_{free}$ to the tree with $x_{p} \in V$ as the new node's parent, i.e. $V \leftarrow V \cup \{x_{n} \}; E \leftarrow E \cup \{(x_{p},x_{n}) \}$.

\Procedure{$X_{sol} \leftarrow Solution(x,T)$}
Finds the path through $T$, $X_{sol}$, that leads from the root of the tree to $x \in V$.

\Procedure{$X_{path} \leftarrow Path(x_{start},x_{end})$}
Builds an ordered set of states that connect the state $x_{start} \in X$ to $x_{end} \in X$ without considering obstacles.
Note that $Solution$ is used to search the tree while $Path$ is used to search the configuration space in attempt to grow the tree.

\Procedure{$bool_{collision} \leftarrow CollisionFree(X_{path})$}
Returns true if $X_{path}$ is obstacle free, $X_{path} \subset X_{free}$. It returns false otherwise.

\Procedure{$x_{p} \leftarrow Parent(x_{c},T)$}
Returns the parent node of $x_{c} \in V$ in the tree $T$, or the null set, $\varnothing$, if $x_{c}$ is the root.

\Procedure{$X_{children} \leftarrow Children(x_{p},T)$}
Returns every node from the set $V$ in $T$ that has $x_{p}$ as its parent node.

\Procedure{$c_v \leftarrow Cost(x_{v},T)$}
Returns the cost of $x_{v} \in V$.
The cost of a vertex is defined as the path length traveled from $x_{r}$ to $x_{v}$ along the tree, i.e.
\begin{equation*}
  Cost(x_{v},T) := c(Solution(x_{v},T))
\end{equation*}
%However, the cost of a vertex can be defined based on many factors.
%For example, cost can be defined in part by a cost map, designed to encourage productive tree growth, see \cite{sampling_based_path_planning_on_configuration-space_costmaps}.
%The only hard constraint on the cost function is that it must monotonically increase from parent to child node.
%If this requirement is violated cycles will form in the tree structure \cite{Karaman2011}.

\Procedure{$c_n \leftarrow CostToCome(x_{n},x_{p},T)$}
Calculates the cost of $x_{n} \in X$ if it were connected to the tree through $x_{p} \in V$, returning an infinite cost if the path is not obstacle free. It is defined in in Algorithm \ref{alg:cost_to_come}.

\begin{algorithm}[h]
  \caption{$c_n \leftarrow CostToCome(x_{n},x_{p},T)$}
  \label{alg:cost_to_come}
  $X_{path} \leftarrow Path(x_{p},x_{n})$\; \label{alg:cost_to_come:path}
  \If{$CollisionFree(X_{path})$}
  { \label{alg:cost_to_come:collision_check}
    \Return $Cost(x_{p},T) + c(X_{path})$; \label{alg:cost_to_come:cost}
  }
  \lElse
  {
    \Return $\inf$\!\!
  }
\end{algorithm}

% common_procedures.tex %

